Ressource Efficient Stabilization for Local Tasks despite Unknown Capacity Links

Self-stabilizing protocols enable distributed systems to recover correct behavior starting from any arbitrary configuration. In particular, when processors communicate by message passing, fake messages may be placed in communication links by an adversary. When the number of such fake messages is unknown, self-stabilization may require huge resources: (a) generic solutions (a.k.a. data link protocols) require unbounded resources, which makes them unrealistic to deploy and (b) specific solutions (e.g., census or tree construction) require $O(n\log n)$ or $O(\Delta\log n)$ bits of memory per node, where $n$ denotes the network size and $\Delta$ its maximum degree, which may prevent scalability. We investigate the possibility of resource efficient self-stabilizing protocols in this context. Specifically, we present a self-stabilizing protocol for $(\Delta+1)$-coloring in any n-node graph, under the asynchronous message-passing model. It is deterministic, it converges in $O(k\Delta n^2\log n)$ message exchanges, where $k$ is the bound of the link capacity in terms of number of messages, and it uses messages on $O(\log\log n+\log\Delta)$ bits with a memory of $O(\Delta\log\Delta+\log\log n)$ bits at each node. The resource consumption of our protocol is thus almost oblivious to the number of nodes, enabling scalability. Moreover, a striking property of our protocol is that the nodes do not need to know the number, or any bound on the number of messages initially present in each communication link of the initial (potentially corrupted) network configuration. This permits our protocol to handle any future network with unknown message capacity communication links. A key building block of our coloring scheme is a spanning directed acyclic graph construction, that is of independent interest, and can serve as a useful tool for solving other tasks in this challenging setting.

==> OldColor.tex <==
\section{Coloring Algorithm}




\begin{theorem}
\label{theo}
There exists a deterministic self-stabilizing protocol that solves $(\Delta+1)$-coloring in any $n$-node graph with maximum degree~$\Delta$, under the asynchronous message-passing model. The protocol uses messages on $O(\log \Delta)$ bits, and a memory of $O(\Delta \log \Delta+\log \log n)$ bits at each node. It converges after $O(km\log n)$ message receptions, where $k$ is the maximum number of (potentially corrupted) messages initially present in each communication link. The value of $k$ does not need to be known by the protocol. 
\end{theorem}

We prove this theorem by designing and analysis a protocol, referred as Algorithm \AlgoC\/ in the rest of the paper, which offers the properties specified in the statement of Theorem~\ref{theo}. This algorithm includes specific techniques for handling spurious initial messages without relying on a data link layer, which might be of general interest, beyond the coloring task. This is the first compact self-stabilizing protocol in the (fully) asynchronous massage-passing model where no bounds on the number of messages initially occupying the communication links need to be given to the nodes. 
%%%%%%

\subsection{Informal description of our algorithm}
Let us present now an informal description of our solution. Our algorithm is given an formal way in Algorithm~\AlgoC. A node $v$ is going to exchange permanently its color with its neighbors. 
 To achieve that $v$ use a message composed of two values. 
 More precisely, $v$ sends its color $\clr_v$ and the color which it knows of its neighbor $u$ stored in variable $\know_v[\port(v,u)]$. 
In non erroneous execution, the node $v$ sends $(\clr_v,\clr_u)$. 

When there exist at least one neighbor $u$ with the same color of $v$, one of them must change its color, to achieve that the node $v$ checks its label by using the function $\Label(\cnt_v,\ID_v)$.
If this function returns $1$, the node $v$ does not change its color. 
Otherwise $v$ changes its color for the \lelia{minimum color available in the set of colors that it knows of its neighbors. 
To achieve this, the node $v$ computes the minimum value stored in the array $\Col_{v}$, this array stores the colors that $v$ knows of its neighbors.  }
The main idea is to reach a configuration where two neighbors $u$ and $v$ with the same color have a different bit returned by their respective label function.
A node $v$ that receives at least one message $(\clr_v,\clr_v)$ by its neighbor $u$ can conclude that its neighbor $u$ has the same color of it, namely  $u$ and $v$ are in conflict.
At the reception of the message  $(\clr_v,\clr_v)$, the node $v$ checks the function  $\Label(\cnt_v,\ID_v)$ if the function returns $1$, it sends at the node in conflict $(\clr_v,\clr_v)$ otherwise the node $v$ changes its color for $\clr'$ and sends $(\clr',\bot)$, in the both cases $v$ increases its counter $\cnt_v$.
 
Unfortunately, there exist two main difficulties related to the channels of communications we must overcome. 
First, we need to manage the existence of erroneous messages in the initial configuration, we bounded this number by an integer $k$. Remember that we do not know $k$, that avoids a simple way to manage these erroneous messages.
As well as, the presence of empty channels of communication, that implies the use of procedure \emph{Do forever},  procedure injecting new messages. 
If we do not manage correctly the use of \emph{Do forever}, we can create a circular reading of the bits of the labels, namely an asynchronous reading between the labels of two neighbors. 
That means, due to the procedure \emph{Do forever} we can obtain a different number of messages between to neighbors $u$ and $v$, and the scheduler can manage this number to create symmetric reading forever.

To overcome the presence of erroneous messages in the initial configuration, we create an acknowledgment. When a node $v$ received the color $\clr_u$ of its neighbor $u$ in message $m$,  for validated $\clr_u$ and put this color in $\Col_v[\port(v,u)]$, the node $v$ must receive its own color in the same time, namely in message $m$. Moreover, when a node changes its color, it deletes the knowledge that its neighbors have of itself. 

To overcome the collateral damage caused by the necessary use of procedure \emph{Do forever}, we used a boolean variable denoted by $\state_v$.
A node $v$ which has its incoming channel with $u$ empty can use the procedure \emph{Do forever}. 
The result of the use of the procedure \emph{Do forever} is the sending of a message $\bot$ to $u$. 
When $u$  receives this message $\bot$ it sends a new message $(\clr_u,\bot)$ and it changes its state. 
But a node $v$ can use several times \emph{Do forever} as a result the sending of several messages $\bot$. 
This several messages could create a sequence of several messages $(\clr_u,\bot)$ which could be used by the scheduler to create an asynchronous reading of the labels of $u$ and $v$.
In the purpose to avoid this, when $u$ receives the first message $\bot$, $u$ it changes its state, so at the receives the other messages $u$ does nothing.


\subsection{Identifiers and Labels}
To break symmetric states between two nodes we use the identifiers, in fact, we do not use directly the identifier, we used a label which is a modification of the identifier.
We use the label introduced by \cite{BournatDD16}, more precisely, each bit of the binary representation of the identifier is duplicated and the bits ''101''  are added at the end of the sequence of these duplicated bits.  
These labels assure for two nodes $v$ and $u$, the label of $u$ is not a prefix of the label of $v$ and vice-versa~\cite{BournatDD16}, even if the lecture of the label is not started at the same place on the label.  
Note that, we do not store the label for a node $v$, this label is recomputed at each time of the algorithm of $v$ needs it, as the consequence, it is not stored in the memory.
 A node $v$ reads its label bit by bit. To achieve that $v$ uses a variable counter $\cnt_{v}$ when the counter achieves the reading of the last bit of the label (in other words, the counter reaches $2\lceil \log \ID(v)\rceil+3$) then the node $v$ restarts its counter. 

For example, suppose node $v$ has identifier $11$ (in decimal notation), or $1011$ (in binary notation), so its label is $\ell(v)=11001111010$. Then, one can implement $\Label(v,i)$ as follows ($i$ is called index):
$$
\Label(v,i) := \left\{
\begin{tabular}{lll}
1 &if &i=1\\
1 &if& i=2\\
0 &if& i=3\\
\dots &if& i=\dots\\
1 &if& i=10\\
0 &if& i=11\\
\end{tabular}
\right.
$$
Since we assume that all identifiers  are $O(\log n)$ bits long, the variable counter  requires $O(\log\log n)$ bits of memory.  
In our algorithm if two neighbors $u$ and $v$ have the same color, they compare their label bit by bit, if the function $\Label(\ID_u,\cnt_u)$ returns $1$ the node $u$ does not change its color, otherwise $u$ changes its color.



==> preuveseb.tex <==
\begin{proof}
  Consider that there exists an infinite execution $e= \gamma_1, \gamma_2, \gamma_3,\ldots$ such that there exists a node $u$ that changes its color infinitely often in $e$. Since nodes have finite memory, channels have finite capacity $k$ (unkown to the nodes), and messages have finite domain, configurations appearing in $e$ form a finite set. As $e$ is infinite, there exists an index $i$ such that after configuration $\gamma_i$, only reccurring configurations appear in $e$ (that is, only configurations that appear infinitely often in $e$ remain). Let $e_i$ denote the suffix of $e$ starting from $\gamma_i$. In $e_i$, node $u$ changes its color infinitely often, so there exists two configurations $\gamma_\alpha$ and $\gamma_\beta$ appearing in $e_i$ such that $u$'s color is different in $\gamma_\alpha$ and in $\gamma_\beta$.
  
 Now, let $j$ denote the first index such that between $\gamma_i$ and $\gamma_j$, all reccurring configurations in $e_i$ appear at least once, and $\gamma_i = \gamma_j$. Let $e_{[i,j[}$ denote the execution fragment starting in $\gamma_i$ and stopping just before $\gamma_j$. Since all reccuring configurations in $e_i$ are present in $e_{[i,j[}$, in particular $\gamma_\alpha$ and $\gamma_\beta$ are present in $e_{[i,j[}$. So, node $u$ changes its color at least once in $e_{[i,j[}$. Now, consider the execution $e'$ formed by $e_{[i,j[}$,$e_{[i,j[}$,$\ldots$ This execution is periodic, and $u$ changes its color infinitely often in $e'$.
\end{proof}

